Towards LLM Unlearning Resilient to Relearning Attacks: A Sharpness-Aware Minimization Perspective and Beyond

The LLM unlearning technique has recently been introduced to comply with data regulations and address the safety and ethical concerns of LLMs by removing the undesired data-model influence. However, state-of-the-art unlearning methods face a critical vulnerability: they are susceptible to ``relearning'' the removed information from a small number of forget data points, known as relearning attacks. In this paper, we systematically investigate how to make unlearned models robust against such attacks. For the first time, we establish a connection between robust unlearning and sharpness-aware minimization (SAM) through a unified robust optimization framework, in an analogy to adversarial training designed to defend against adversarial attacks. Our analysis for SAM reveals that smoothness optimization plays a pivotal role in mitigating relearning attacks. Thus, we further explore diverse smoothing strategies to enhance unlearning robustness. Extensive experiments on benchmark datasets, including WMDP and MUSE, demonstrate that SAM and other smoothness optimization approaches consistently improve the resistance of LLM unlearning to relearning attacks. Notably, smoothness-enhanced unlearning also helps defend against (input-level) jailbreaking attacks, broadening our proposal's impact in robustifying LLM unlearning. Codes are available at https://github.com/OPTML-Group/Unlearn-Smooth.

==> sections/experiments.tex <==
%\newpage
\section{Experiments}
\label{sec: exp}
\subsection{Experiment setups}
\textbf{Datasets and models.} To showcase the robustness improvements brought by SAM and other smoothing techniques, we perform experiments on two representative benchmarks:
 \textbf{(1) WMDP} \cite{li2024wmdp}, as used in Fig.\,\ref{fig: NPO_example}, which evaluates the unlearning capability and knowledge retention of LLMs in hazardous domains, such as biosecurity, cybersecurity, and chemical security. Our experiments primarily focus on the biosecurity aspect of WMDP; 
 \textbf{(2) MUSE} \cite{shi2024muse}, which features two distinct unlearning scenarios: forgetting text segments from the Harry Potter book series (labeled `Books') and forgetting news articles from BBC News (labeled `News').
\SL{We use xxx as the original pre-unlearning model (referred to as `Origin' in Fig.\,\ref{fig: NPO_example}).} 
%For the MUSE benchmark, the original model was fine-tuned on the Books and News datasets for knowledge memorization.
 \SL{[missing model information.]}
  

\textbf{LLM unlearning methods and evaluation.} 
%In our experiments, we selected several important and state-of-the-art (SOTA) methods as baselines to demonstrate the robustness improvements provided by SAM and other smoothing techniques. We denote the model before any unlearning operations as \textbf{Original}. Specifically, for WMDP, \textbf{Original} refers to the pre-trained model without fine-tuning on any specific dataset. In contrast, for MUSE, \textbf{Original} is the model fine-tuned on the respective Books or News datasets. 
%
%Starting from this \textbf{Original} model, we apply a variety of unlearning methods to the designated “forget” and “retain” sets to achieve the unlearning objective described in Equation~\eqref{eq: prob_LLM_MU}.
For the WMDP benchmark, we use NPO \cite{zhang2024negative} with retain regularization as the primary unlearning baseline, as formulated by  \eqref{eq: prob_LLM_MU}. Additionally, we include Representation Misdirection for Unlearning (RMU) \cite{li2024wmdp} and Gradient Difference (GradDiff) \cite{maini2024tofu,liu2022continual} as supplementary baselines. For   MUSE, we adopt NPO as the baseline due to its state-of-the-art (SOTA) performance on this benchmark \cite{shi2024muse}.
%
More implementation details are provided in Appendix\,\ref{appendix: exp_setup}.

Following the used benchmarks, the performance of LLM unlearning is evaluated by \textbf{UE} (unlearning effectiveness) and post-unlearning model utility (\textbf{UT}). For WMDP, UE is measured as 1-Accuracy on the WMDP Bio evaluation set, consistent with Fig.\,\ref{fig: NPO_example}. UT is assessed using zero-shot accuracy on the MMLU dataset \cite{hendrycks2020measuring}.
For MUSE, UE is evaluated based on knowledge memorization ({KnowMem}) and  verbatim memorization ({VerbMem}) on the forget set,  where lower values indicate better unlearning performance.
\SL{[UT in MUSE is missing?]}
In addition to UE and UT, we assess the \textbf{robustness} of LLM unlearning in two adversarial settings: \textbf{relearning attacks} \cite{hu2024jogging}, which is our primary focus; And \textbf{jailbreaking attacks} \cite{lucki2024adversarial, thompson2024flrt}, given by input-level adversaries that craft adversarial prompts to extract unlearned information from an unlearned model without modifying its parameters.
To implement  relearning attacks, we sample relearning data from either the forget set or an unrelated dataset, such as AGNews, GSM8K, or SST2. For  jailbreaking attack, we use the enhanced-GCG algorithm \cite{lucki2024adversarial,zou2023universal,thompson2024flrt} to generate adversarial prefixes.










% \ding{182} \textbf{Unlearning Effectiveness} measures the extent to which undesired data influences or model capabilities are removed. For WMDP, we use \textbf{1 - WMDP Bio Accuracy} as the metric, where a higher value indicates better unlearning. For MUSE, we evaluate using knowledge memorization (\textbf{KnowMem}) and  verbatim memorization (\textbf{VerbMem}) on the forget set $\mathcal{D}_f$; lower values are better. 
% \ding{183} \textbf{Utility Retention} assesses the preserved capabilities of the unlearned model. This is evaluated by the zero-shot accuracy on the \textbf{MMLU} dataset \cite{hendrycks2020measuring} within the WMDP benchmark. 

%\ding{184} \textbf{Robustness} evaluates the resilience of the unlearned model against relearning attacks \cite{hu2024jogging} and jailbreaking attacks\cite{lucki2024adversarial, thompson2024flrt}. The attack settings and detailed evaluation protocols are described in the following paragraph.

% \textbf{Attacks to LLM unlearning.}
% For the \textbf{Relearning attack}, we sample a small number of examples from a given dataset. Specifically, we consider two attack settings: \textit{(S1) the fixed number of samples which is randomly sampled from the given set, and conduct relearning on these samples with different numbers of relearning epochs}, and \textit{(S2) different numbers of relearning samples randomly sampled from given dataset and relearning on these samples for one epoch}. For WMDP, we use different relearning sets by sampling from the WMDP Bio forget set, AGNews, GSM8K, and SST2. In the case of (S1), we sample 20 examples and perform relearning for 1, 2, and 3 epochs, respectively. For (S2), we sample 20, 40, and 60 examples and perform relearning for 1 epoch, respectively. For MUSE, We sample 100, 125, and 150 examples from the forget set as the relearning set and conduct relearning for one epoch. \textbf{For the adversarial prompt}, we follow the setup in \cite{lucki2024adversarial,thompson2024flrt}, using Enhanced-GCG to generate adversarial prefixes, which are then combined with the WMDP Bio evaluation set for evaluation.




For the \textbf{Relearning attack}, we sample a small number of examples from a given dataset. Specifically, we consider two attack settings:
\textit{(S1) Fixed Number of Samples:} A fixed number of samples are randomly selected from the given set, and relearning is conducted on these samples with varying numbers of relearning epochs.
\textit{(S2) Varying Number of Samples:} Different numbers of relearning samples are randomly selected from the given dataset, and relearning is performed on these samples for a single epoch. For the WMDP benchmark, we create different relearning sets by sampling from the WMDP Bio forget set, AGNews, GSM8K, and SST2 datasets: In setting \textit{(S1)}, we sample 20 examples and perform relearning for 1, 2, and 3 epochs, respectively. In setting \textit{(S2)}, we sample 20, 40, and 60 examples and perform relearning for 1 epoch each. For the MUSE benchmark, we adopt setting \textit{(S2)} and sample 100, 125, and 150 examples from the forget set as the relearning set, conducting relearning for one epoch. As for the robustness against \textbf{jailbreaking attacks}, we follow the setup in \cite{lucki2024adversarial,thompson2024flrt}, using Enhanced-GCG to generate adversarial prefixes, which are then combined with the WMDP Bio evaluation set for evaluation.



\subsection{Robustness against relearning attacks on WMDP.}

% \textbf{Robustness against relearning attacks with different epochs.} Following \textit{(S1)}, we fixed the number of relearning samples at 20 and progressively increased the number of relearning epochs. The results are shown in \textbf{Fig.\,\ref{fig: relearn_wmdp_npo}-(a)}. It showcases that SAM significantly reduces the rate of decline in 1 - WMDP Bio Acc compared with NPO, which represents that SAM can significant slow down the speed of relearning knowledge back on WMDP datasets compared with NPO. Specifically, unlearning effectiveness of NPO+SAM at epoch 3 have 0.2 improvement compared with NPO. In contrast, for NPO, relearning with just 20 samples for a single epoch already causes a substantial drop in 1 - WMDP Bio Acc. After 3 epochs of relearning, the model's performance nearly converges to that of the original model, effectively invalidating the unlearning process. Besides, we can also observe that other smoothing techiques also can improve the robustness in this relearning attack settings but not competitive as SAM, which is reasonable, because from the \eqref{eq: prob_LLM_MU_SAM}, SAM is directly solving the robustness against relearning attack problem. 


\textbf{Robustness against relearning attacks with different epochs.} Following the \textit{(S1)} attack setting, we fixed the number of relearning samples at 20 and progressively increased the number of relearning epochs. The results are presented in \textbf{Fig.\,\ref{fig: relearn_wmdp_npo}-(a)}. The figure demonstrates that integrating SAM with NPO during unlearning significantly reduces the rate of decline in $1 - \text{WMDP Bio Acc}$ as relearning epochs increasing . This indicates that integrating SAM with NPO can significantly slow down the speed at which knowledge is relearned on the WMDP dataset. Specifically, the unlearning effectiveness of NPO+SAM shows a 0.21 \JH{preciser number} improvement at epoch 3 compared with NPO alone. In contrast, for NPO, relearning with just 20 samples for a single epoch already causes a substantial drop in $1 - \text{WMDP Bio Acc}$. After 3 epochs of relearning, the model's performance nearly converges to that of the original model, effectively invalidating the unlearning process. Additionally, other smoothing techniques also improve robustness consistently under this relearning attack setting, though they are not as competitive as SAM. This is expected, as SAM directly addresses the robustness against relearning attacks, as formulated in Equation~\eqref{eq: prob_LLM_MU_SAM}. It can be observed that SAM and GP are the most effective among the four smoothing methods, significantly enhancing NPO’s robustness against relearning attacks.



\begin{figure}[htb]
\begin{tabular}{cc}
\hspace*{-3mm}
\includegraphics[width=0.24\textwidth,height=!]{figs/npo_epoch_wmdp_var.pdf} 
&
\hspace*{-3mm}
\includegraphics[width=0.24\textwidth,height=!]{figs/npo_step_wmdp_var.pdf}
\vspace*{-1mm}
\\
\hspace*{3mm} \small{(a) Relearning setting \textit{(s1)}} & 
 \small{(b) Relearning setting \textit{(s2)}}\\
% \hspace*{2mm} {(a) Forget quality} & {(b) Model utility}
\end{tabular}
% }
\vspace{-2mm}
\caption{\small{Performance of relearning attacks on the WMDP Bio dataset across various unlearning approaches under two different relearning attack settings. \textbf{(a)} The number of relearning samples is fixed at 20, while the number of relearning epochs varies (1, 2, 3). \textbf{(b)} The number of relearning epochs is fixed at 1, while the number of relearning samples varies (20, 40, 60). Unlearning effectiveness is measured as 1 - WMDP Bio accuracy, where higher values indicate better unlearning performance. Results are averaged over five independent random trials.}}
\label{fig: relearn_wmdp_npo}
\vspace*{-2mm}
\end{figure}

\textbf{Robustness against relearning attacks with increasing samples.} Following the \textit{(S2)} attack setting, we fixed the number of relearning epochs to 1 and progressively increased the number of relearning samples. The results are presented in \textbf{Fig.\,\ref{fig: relearn_wmdp_npo}-(b)}. The figure demonstrates that integrating SAM with NPO during unlearning reduces the rate of decline in $1 - \text{WMDP Bio Acc}$  as the number of relearning samples increasing. However, compared to the results in \textit{(S1)}, the benefit provided by SAM is less significant. This suggests that using a larger number of relearning samples with fewer relearning epochs constitutes a stronger relearning attack than using a smaller number of samples with more epochs. Additionally, we observe a same order of robustness across different smoothing techniques combined with NPO in the relearning attacks under \textit{(S1)}, and they all consistently enhance the robustness of NPO.

\begin{table*}[t]
\caption{Performance overview of different NPO variants, with and without various smoothing techniques, on the WMDP Bio benchmark \cite{li2024wmdp} across multiple relearning datasets, including WMDP Bio \cite{li2024wmdp}, AGNews \cite{zhang2015character}, GSM8K \cite{cobbe2021gsm8k}, and SST2 \cite{socher2013recursive}. An upward arrow (\textuparrow) indicates that higher metric values signify better performance. The performance gap in WMDP Bio Accuracy before and after the relearning attack is denoted by (\textcolor{blue}{$\bullet$}). A smaller performance gap compared to the \textit{"Before Attack"} accuracy reflects better robustness of the MU method. The \textit{Avg.} metric represents the average of $1 - \text{WMDP Bio Acc}$ across the WMDP Bio, AGNews, GSM8K, and SST2 datasets.}
\label{tab: relearn_wmdp}
\begin{center}
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{c|c|c|cccc|c}
\toprule[1pt]
\midrule
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{MMLU (\textuparrow)} & \multicolumn{6}{c}{1 - WMDP Bio Acc (\textuparrow)} \\                             
\cmidrule{3-8}
& & Before Attack & WMDP Bio & AGNews & GSM8K & SST2 & Avg. \\
\midrule
\rowcolor{Gray}
\multicolumn{8}{c}{\textbf{(S1) 20 samples for 3 epochs}} \\
\midrule
NPO       & 0.44 & 0.74 & 0.37 (\textcolor{blue}{0.37}) & 0.39 (\textcolor{blue}{0.35}) & 0.38 (\textcolor{blue}{0.36}) & 0.38 (\textcolor{blue}{0.36}) & 0.38 (\textcolor{blue}{0.36}) \\
\midrule
NPO + SAM & 0.42 & 0.74 & 0.59 (\textcolor{blue}{0.15}) & 0.41 (\textcolor{blue}{0.33}) & 0.42 (\textcolor{blue}{0.32}) & 0.41 (\textcolor{blue}{0.32}) & 0.46 (\textcolor{blue}{0.28}) \\
NPO + RS  & 0.41 & 0.74 & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.33}) & 0.42 (\textcolor{blue}{0.32}) \\
NPO + CR & 0.43 & 0.75 & 0.52 (\textcolor{blue}{0.23}) & 0.4 (\textcolor{blue}{0.34})  & 0.55 (\textcolor{blue}{0.2})  & 0.43 (\textcolor{blue}{0.32}) & 0.47 (\textcolor{blue}{0.27}) \\
NPO + GP & 0.45 & 0.73 & 0.43 (\textcolor{blue}{0.30}) & 0.40 (\textcolor{blue}{0.33}) & 0.45 (\textcolor{blue}{0.28}) & 0.49 (\textcolor{blue}{0.24}) & 0.44 (\textcolor{blue}{0.29}) \\
NPO + WA & 0.46 & 0.74 & 0.43 (\textcolor{blue}{0.30}) & 0.39 (\textcolor{blue}{0.34}) & 0.39 (\textcolor{blue}{0.35}) & 0.39 (\textcolor{blue}{0.34}) & 0.40 (\textcolor{blue}{0.33}) \\
\midrule
\rowcolor{Gray}
\multicolumn{8}{c}{\textbf{(S2) 60 samples for 1 epoch}} \\
\midrule
NPO       & 0.44 & 0.74 & 0.37 (\textcolor{blue}{0.37}) & 0.39 (\textcolor{blue}{0.35}) & 0.37 (\textcolor{blue}{0.37}) & 0.38 (\textcolor{blue}{0.36}) & 0.38 (\textcolor{blue}{0.36}) \\
\midrule
NPO + SAM & 0.42 & 0.74 & 0.45 (\textcolor{blue}{0.29}) & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.32}) & 0.43 (\textcolor{blue}{0.31}) & 0.43 (\textcolor{blue}{0.31}) \\
NPO + RS  & 0.41 & 0.74 & 0.41 (\textcolor{blue}{0.33}) & 0.41 (\textcolor{blue}{0.33}) & 0.41 (\textcolor{blue}{0.33}) & 0.40 (\textcolor{blue}{0.34}) & 0.41 (\textcolor{blue}{0.33}) \\
NPO + CR & 0.43 & 0.75 & 0.43 (\textcolor{blue}{0.32}) & 0.41 (\textcolor{blue}{0.34}) & 0.67 (\textcolor{blue}{0.08}) & 0.43 (\textcolor{blue}{0.32}) & 0.48 (\textcolor{blue}{0.26}) \\
NPO + GP & 0.45 & 0.73 & 0.43 (\textcolor{blue}{0.30}) & 0.48 (\textcolor{blue}{0.25}) & 0.50 (\textcolor{blue}{0.23}) & 0.49 (\textcolor{blue}{0.24}) & 0.47 (\textcolor{blue}{0.25}) \\
NPO + WA & 0.46 & 0.74 & 0.40 (\textcolor{blue}{0.34}) & 0.42 (\textcolor{blue}{0.32}) & 0.39 (\textcolor{blue}{0.34}) & 0.40 (\textcolor{blue}{0.34}) & 0.40 (\textcolor{blue}{0.34}) \\
\midrule
\bottomrule[1pt]
\end{tabular}
}
\end{center}
\end{table*}


\textbf{Robustness against relearning attacks with different relearning set.} In addition to only using the WMDP Bio forget set for the relearning attack, we also perform relearning attacks on other datasets, such as AGNews \cite{zhang2015character}, GSM8K \cite{cobbe2021gsm8k}, and SST2 \cite{socher2013recursive}. We consider the same two relearning settings, following \textit{(S1)} and \textit{(S2)}, and report the results of the final model during unlearning (20 samples for 3 epochs or 60 samples for 1 epoch) in \textbf{Table\,\ref{tab: relearn_wmdp}}. Across all datasets, the gap caused by the relearning attack is consistently smaller for NPO+SAM compared to NPO alone. And we can get similar observation that SAM and GP are two most effective smoothing techniques that improve robustness of NPO. 

\begin{figure}[htb]
% \vspace*{-5mm}
\begin{tabular}{cc}
\hspace*{-3mm}
\includegraphics[width=0.24\textwidth,height=!]{figs/method_epoch_wmdp_var.pdf} 
&
\hspace*{-3mm}
\includegraphics[width=0.24\textwidth,height=!]{figs/method_step_wmdp_var.pdf}
\vspace*{-1mm}
\\
\hspace*{3mm} \small{(a) Relearning setting (s1)} & 
 \small{(b) Relearning setting (s2)}\\
\end{tabular}
\vspace{-2mm}
\caption{\small{Performance of Relearning Attacks on WMDP Bio for NPO, GradDiff, and RMU w/o or w/ SAM. The figure format follows Fig.\,\ref{fig: relearn_wmdp_npo}.
}}
\label{fig: relearn_wmdp_method}
\vspace*{-5mm}
\end{figure}

% \textbf{Generalization to smoothing method.} {\JH{not sure whether keeping this paragraph or not, we have discussed following in previous subsections}}In Fig.\,\ref{fig: relearn_wmdp_npo}-(a) and (b), we demonstrate the generalizability of NPO to various smoothing methods. We combine NPO with SAM, GNR, RS, and SWA, and evaluate their robustness under two relearning settings, following (S1) and (S2). The results show that incorporating smoothing methods consistently improves the robustness of NPO against relearning attacks. In Table\,\ref{tab: relearn_wmdp}, we present the final results for both (S1) and (S2). It can be observed that SAM and GNR are the most effective among the four smoothing methods, significantly enhancing NPO's robustness against relearning attacks.

\textbf{Robustness Enhancement with SAM Across Different Unlearning Methods.} To demonstrate that SAM can improve robustness not only for the NPO unlearning method but also for other unlearning methods, we conduct experiments by integrating SAM with GradDiff \cite{maini2024tofu} and RMU \cite{li2024wmdp}, as shown in \textbf{Fig.\,\ref{fig: relearn_wmdp_method}-(a)} and \textbf{Fig.\,\ref{fig: relearn_wmdp_method}-(b)}. This showcases the generalizability of SAM across different unlearning methods. Specifically, we combine SAM with NPO, GradDiff, and RMU, and evaluate their robustness under the two relearning settings, \textit{(S1)} and \textit{(S2)}. The results indicate that SAM significantly enhances the robustness of all three methods against relearning attacks, particularly under the \textit{(S1)} setting. Notably, we observe varying levels of robustness among the different methods: NPO exhibits the highest robustness, followed by GradDiff, while RMU shows the weakest robustness. This disparity arises because RMU performs unlearning only on a partial model (layers 5, 6, and 7), whereas the relearning attack targets the full model. Consequently, the mismatch in parameter updating between the unlearning and relearning phases leads to reduced robustness in RMU compared to NPO and GradDiff.



% \textbf{Visualization of loss landscape over forgetting data.} We visualize the prediction loss landscape of the unlearned model over the forgetting data in \textbf{Fig.\,\ref{fig: loss_landscape_df_diff_smooth}}. The loss landscape of NPO shows a sharp spike at the origin, with rapid variations occurring within a very small region. However, when NPO is combined with the smoothing method, the sharp spike disappears, and the variations at the origin become relatively smooth. This smoothness ensures that the unlearned model's loss does not fluctuate dramatically under a relearning attack, making it more robust to such attacks. Additionally, in \textbf{Fig.\,\ref{fig: loss_landscape_dr_diff_smooth} of Appendix\,\ref{appendix: add_exp}}, we show the prediction loss landscape of the unlearned model over the retaining data. These observations demonstrate how the smoothing method enhances the robustness of the unlearning method.

% \begin{itemize}
%     \item Evaluate robustness under two different relearning settings (\textbf{Table\,\ref{tab: relearn_wmdp}} + \textbf{Fig.\,\ref{fig: relearn_wmdp_npo}} + \textbf{Fig.\,\ref{fig: relearn_wmdp_method}} + loss landscape)
%         \begin{itemize}
%             \item Same number of relearning samples but with different relearning epochs.
%             \item Different numbers of relearning samples with the same relearning epoch.
%         \end{itemize} 
%     \item Combining different smoothing methods with unlearning methods improves model robustness.
%     \item Robustness of unlearning method NPO $>$ GradDiff $>$ RMU
% \end{itemize}

\subsection{Performance on the MUSE Benchmark}
\textbf{Generalization to unlearning benchmarks.} We conduct additional experiments on the MUSE News and MUSE Books benchmarks. To evaluate unlearning performance, we use KnowMem on $\mathcal{D}_\mathrm{f}$ and VerbMem on $\mathcal{D}_\mathrm{f}$, where lower values indicate better performance. The results are shown in the figure. It can be observed that combining NPO with SAM reduces the magnitude of decrease in both KnowMem on $\mathcal{D}_\mathrm{f}$ and VerbMem on $\mathcal{D}_\mathrm{f}$, further confirming that SAM enhances robustness against relearning attacks. The complete unlearning performance before the relearning attack is detailed in \textbf{Table\,\ref{tab: relearn_muse}} in \textbf{Appendix\,\ref{appendix: add_result_muse}}. Moreover, we observe that the final changes in VerbMem on $\mathcal{D}_\mathrm{f}$ after the relearning attack are larger than those in KnowMem on $\mathcal{D}_\mathrm{f}$. This phenomenon consistently appears in both MUSE Books and MUSE News, suggesting that words are inherently more vulnerable to relearning attacks compared to knowledge.

\begin{figure}[htb]
\begin{tabular}{cc}
\hspace*{-3mm}
\includegraphics[width=0.23\textwidth,height=!]{figs/muse_books_2d.pdf} 
&
% \hspace*{-6mm}
\includegraphics[width=0.23\textwidth,height=!]{figs/muse_news_2d.pdf}
\vspace*{-1mm}
\\
\hspace*{3mm} \small{(a) MUSE Books} & \small{(b) MUSE News}\\
\end{tabular}
\vspace{-2mm}
\caption{\small{Performance of relearning attacks on MUSE Books and MUSE News for NPO and NPO w/ SAM under setting \textit{S2} \JH{@chongyu attack settings}. Unlearning effectiveness is evaluated using KnowMem on $\mathcal{D}_\mathrm{f}$ and VerbMem on $\mathcal{D}_\mathrm{f}$. Different relearned models are obtained by varying the number of relearning samples while keeping the number of relearning epochs constant. The closer the Relearned model is to the Original model, the less robust it is.}}
\label{fig: relearn_muse_npo}
\vspace*{-5mm}
\end{figure}

\textbf{Ablation Study on SAM's Hyperparameter $\rho$.}
$\rho$ is a hyperparameter in SAM that controls the magnitude of weight perturbation, with larger $\rho$ values corresponding to stronger perturbations. We conduct an ablation study on $\rho$ using the MUSE Books benchmark, and the results are shown in \textbf{Table\,\ref{tab: muse_rho_ablation}} in \textbf{Appendix\,\ref{appendix: add_result_muse}}. It can be observed that when $\rho$ is too small (e.g., $0.001$), SAM provides limited improvement against relearning attacks. Conversely, when $\rho$ is too large (e.g., $0.1$), the perturbations become excessive, preventing the model from successfully unlearning. When $\rho = 0.01$, the model achieves a balance: it successfully unlearns while also demonstrating improved robustness, with smaller changes of KnowMem on $\mathcal{D}_\mathrm{f}$ and VerbMem on $\mathcal{D}_\mathrm{f}$ observed before and after the relearning attack.

\subsection{Robustness to adversarial prompt}
In the previous sections, we demonstrated that SAM and other smoothing methods exhibit robustness against relearning attacks, which can be viewed as a type of weight-space attack. In this section, we investigate alternative forms of attacks, particularly those based on the input space, such as adversarial prompts. Specifically, we use Enhanced GCG to generate adversarial prompts \cite{lucki2024adversarial}, which are then combined with questions from the WMDP Bio evaluation set to measure performance. The results indicate that perturbation-based approaches, such as SAM and RS, show strong resilience against adversarial prompts, effectively neutralizing input-space attacks. Other smoothing methods also offer moderate improvements in defending against adversarial prompts.

\begin{table}[htb]
\caption{\small{Performance overview of NPO variants with or without variant smoothing techniques against jailbreaking attacks. The table format follows Table\,\ref{tab: relearn_wmdp}.}}
\label{tab: adv_prompt_wmdp}
\begin{center}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c|c|cc}
\toprule[1pt]
\midrule
\multirow{3}{*}{Method} & \multirow{3}{*}{MMLU (\textuparrow)} & \multicolumn{2}{c}{1 - WMDP Bio Acc (\textuparrow)} \\                        
\cmidrule{3-4}
& & Before Attack & After Attack \\
\midrule
NPO       & 0.44 & 0.74 & 0.45 (\textcolor{blue}{0.29}) \\
\midrule
NPO + SAM & 0.42 & 0.74 & 0.73 (\textcolor{blue}{0.01}) \\
NPO + RS  & 0.41 & 0.74 & 0.74 (\textcolor{blue}{0.00}) \\
NPO + CR  & 0.43 & 0.75 & 0.63 (\textcolor{blue}{0.12}) \\
NPO + GNR & 0.45 & 0.73 & 0.53 (\textcolor{blue}{0.20}) \\
NPO + SWA & 0.46 & 0.74 & 0.47 (\textcolor{blue}{0.27}) \\
\midrule
\bottomrule[1pt]
\end{tabular}
}
\end{center}
\end{table}

% \begin{table}[htb]
% \caption{Unlearning and Relearning Performance on WMDP Bio. Relearning attacks are conducted using WMDP Bio, AGNews, GSM8K, and SST2. \textuparrow indicates that the higher the metric, the better. The performance gap in WMDP Bio Acc before and after the relearning attack is indicated by (\textcolor{blue}{$\bullet$}). Note that a smaller performance gap compared to the \textit{"Before Attack"} accuracy reflects better robustness of the MU method. The metric \textit{Avg.} is calculated as the average 1 - WMDP Bio Acc, including WMDP Bio, AGNews, GSM8K, and SST2.}
% \label{tab: relearn_wmdp}
% \begin{center}
% \resizebox{0.8\columnwidth}{!}{
% \begin{tabular}{c|c|cc}
% \toprule[1pt]
% \midrule
% \multirow{3}{*}{Method} & \multirow{3}{*}{MMLU (\textuparrow)} & \multicolumn{2}{c}{1 - WMDP Bio Acc (\textuparrow)} \\                        
% \cmidrule{3-4}
% & & Before Attack & After Attack \\
% \midrule
% NPO       & 0.44 & 0.74 & 0.45 (\textcolor{blue}{0.29}) \\
% \midrule
% NPO + SAM & 0.42 & 0.74 & 0.73 (\textcolor{blue}{0.01}) \\
% NPO + RS  & 0.41 & 0.74 & 0.74 (\textcolor{blue}{0.00}) \\
% NPO + GNR & 0.45 & 0.73 & 0.53 (\textcolor{blue}{0.20}) \\
% NPO + SWA & 0.46 & 0.74 & 0.47 (\textcolor{blue}{0.27}) \\
% \midrule
% \bottomrule[1pt]
% \end{tabular}
% }
% \end{center}
% \end{table}



% \begin{table*}[t]
% \caption{Unlearning and Relearning Performance on WMDP Bio. Relearning attacks are conducted using WMDP Bio, AGNews, GSM8K, and SST2. \textuparrow indicates that the higher the metric, the better. The performance gap in WMDP Bio Acc before and after the relearning attack is indicated by (\textcolor{blue}{$\bullet$}). Note that a smaller performance gap compared to the \textit{"Before Attack"} accuracy reflects better robustness of the MU method. The metric \textit{Avg.} is calculated as the average 1 - WMDP Bio Acc, including WMDP Bio, AGNews, GSM8K, and SST2.}
% \label{tab: relearn_wmdp}
% \begin{center}
% \begin{tabular}{c|c|c|cccc|c}
% \toprule[1pt]
% \midrule
% \multirow{3}{*}{Method} & \multirow{3}{*}{MMLU (\textuparrow)} & \multicolumn{6}{c}{1 - WMDP Bio Acc (\textuparrow)} \\                             
% \cmidrule{3-8}
% & & Before Attack & WMDP Bio & AGNews & GSM8K & SST2 & Avg. \\
% \midrule
% \rowcolor{Gray}
% \multicolumn{8}{c}{\textbf{(S1) 20 samples for 3 epochs}} \\
% \midrule
% NPO       & 0.44 & 0.74 & 0.37 (\textcolor{blue}{0.37}) & 0.39 (\textcolor{blue}{0.35}) & 0.38 (\textcolor{blue}{0.36}) & 0.38 (\textcolor{blue}{0.36}) & 0.38 (\textcolor{blue}{0.36}) \\
% \midrule
% NPO + SAM & 0.42 & 0.74 & 0.59 (\textcolor{blue}{0.15}) & 0.41 (\textcolor{blue}{0.33}) & 0.42 (\textcolor{blue}{0.32}) & 0.41 (\textcolor{blue}{0.32}) & 0.46 (\textcolor{blue}{0.28}) \\
% NPO + RS  & 0.41 & 0.74 & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.33}) & 0.42 (\textcolor{blue}{0.32}) \\
% NPO + GNR & 0.45 & 0.73 & 0.43 (\textcolor{blue}{0.30}) & 0.40 (\textcolor{blue}{0.33}) & 0.45 (\textcolor{blue}{0.28}) & 0.49 (\textcolor{blue}{0.24}) & 0.44 (\textcolor{blue}{0.29}) \\
% NPO + SWA & 0.46 & 0.74 & 0.43 (\textcolor{blue}{0.30}) & 0.39 (\textcolor{blue}{0.34}) & 0.39 (\textcolor{blue}{0.35}) & 0.39 (\textcolor{blue}{0.34}) & 0.40 (\textcolor{blue}{0.33}) \\
% \midrule
% \rowcolor{Gray}
% \multicolumn{8}{c}{\textbf{(S2) 60 samples for 1 epoch}} \\
% \midrule
% NPO       & 0.44 & 0.74 & 0.37 (\textcolor{blue}{0.37}) & 0.39 (\textcolor{blue}{0.35}) & 0.37 (\textcolor{blue}{0.37}) & 0.38 (\textcolor{blue}{0.36}) & 0.38 (\textcolor{blue}{0.36}) \\
% \midrule
% NPO + SAM & 0.42 & 0.74 & 0.45 (\textcolor{blue}{0.29}) & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.32}) & 0.43 (\textcolor{blue}{0.31}) & 0.43 (\textcolor{blue}{0.31}) \\
% NPO + RS  & 0.41 & 0.74 & 0.41 (\textcolor{blue}{0.33}) & 0.41 (\textcolor{blue}{0.33}) & 0.41 (\textcolor{blue}{0.33}) & 0.40 (\textcolor{blue}{0.34}) & 0.41 (\textcolor{blue}{0.33}) \\
% NPO + GNR & 0.45 & 0.73 & 0.43 (\textcolor{blue}{0.30}) & 0.48 (\textcolor{blue}{0.25}) & 0.50 (\textcolor{blue}{0.23}) & 0.49 (\textcolor{blue}{0.24}) & 0.47 (\textcolor{blue}{0.25}) \\
% NPO + SWA & 0.46 & 0.74 & 0.40 (\textcolor{blue}{0.34}) & 0.42 (\textcolor{blue}{0.32}) & 0.39 (\textcolor{blue}{0.34}) & 0.40 (\textcolor{blue}{0.34}) & 0.40 (\textcolor{blue}{0.34}) \\
% \midrule
% \bottomrule[1pt]
% \end{tabular}
% \end{center}
% \end{table*}

% % \begin{figure}[htb]
% % % \vspace*{-5mm}
% % \resizebox{\columnwidth}{!}{
% %     \includegraphics[width=0.28\columnwidth]{figs/npo_step_wmdp_var.pdf}
% %     \includegraphics[width=0.28\columnwidth]{figs/npo_epoch_wmdp_var.pdf}

% % }
% % \vspace*{-6.5mm}
% % \caption{Performance of Relearning Attacks on NPO w/o or w/ Smoothing. The evaluation is conducted under two relearning settings: (a) varying the number of relearning samples (20, 40, 60) with the same number of relearning epochs (1), and (b) fixing the number of relearning samples (20) while varying the number of relearning epochs (1, 2, 3). The results are averaged over five independent random trials.
% % }
% % % \vspace*{-5mm}
% % \label{fig: relearn_wmdp_npo}
% % \end{figure}

% \begin{figure}[htb]
% % \vspace*{-5mm}
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{cc}
% \hspace*{-3mm}
% \includegraphics[width=0.25\textwidth,height=!]{figs/npo_epoch_wmdp_var.pdf} 
% &
% \hspace*{-6mm}
% \includegraphics[width=0.25\textwidth,height=!]{figs/npo_step_wmdp_var.pdf}
% \vspace*{-1mm}
% \\
% \hspace*{3mm} \small{(a)} & \hspace*{6mm} \small{(b)}\\
% % \hspace*{2mm} {(a) Forget quality} & {(b) Model utility}
% \end{tabular}
% % }
% \vspace{-2mm}
% \caption{\small{Performance of Relearning Attacks on WMDP Bio for NPO w/o or w/ Smoothing. The evaluation is conducted under two relearning settings: (a) fixing the number of relearning samples (20) while varying the number of relearning epochs (1, 2, 3), and (b) varying the number of relearning samples (20, 40, 60) with the same number of relearning epochs (1). The results are averaged over five independent random trials.}}
% \label{fig: relearn_wmdp_npo}
% \vspace*{-5mm}
% \end{figure}


% \begin{figure}[htb]
% % \vspace*{-5mm}
% \begin{tabular}{cc}
% \hspace*{-3mm}
% \includegraphics[width=0.25\textwidth,height=!]{figs/method_epoch_wmdp_var.pdf} 
% &
% \hspace*{-6mm}
% \includegraphics[width=0.25\textwidth,height=!]{figs/method_step_wmdp_var.pdf}
% \vspace*{-1mm}
% \\
% \hspace*{3mm} \small{(a)} & \hspace*{3mm} \small{(b)} \\
% % \hspace*{2mm} {(a) Forget quality} & {(b) Model utility}
% \end{tabular}
% \vspace{-2mm}
% \caption{\small{Performance of Relearning Attacks on WMDP Bio for NPO, GradDiff, and RMU w/o or w/ SAM. The figure format follows Fig.\,\ref{fig: relearn_wmdp_method}.
% }}
% \label{fig: relearn_wmdp_method}
% \vspace*{-5mm}
% \end{figure}


% \begin{figure}[htb]
% % \vspace*{-5mm}
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{cc}
% \hspace*{-3mm}
% \includegraphics[width=0.23\textwidth,height=!]{figs/muse_books_2d.pdf} 
% &
% % \hspace*{-6mm}
% \includegraphics[width=0.23\textwidth,height=!]{figs/muse_news_2d.pdf}
% \vspace*{-1mm}
% \\
% \hspace*{3mm} \small{(a) MUSE Books} & \small{(b) MUSE News}\\
% \end{tabular}
% \vspace{-2mm}
% \caption{\small{Performance of Relearning Attacks on MUSE Books/News for NPO and NPO w/ SAM. Robustness is evaluated using KnowMem on $\mathcal{D}_\mathrm{f}$ and VerbMem on $\mathcal{D}_\mathrm{f}$. Different Relearned models are obtained by varying the number of relearning samples while keeping the number of relearning epochs constant. The closer the Relearned model is to the Original model, the less robust it is.}}
% \label{fig: relearn_muse_npo}
% \vspace*{-5mm}
% \end{figure}


% \begin{figure}[htb]
% % \vspace*{-5mm}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{cc}
% \hspace*{-3mm}
% \includegraphics[width=0.24\columnwidth,height=!]{figs/npo_df.pdf} 
% &
% \hspace*{-6mm}
% \includegraphics[width=0.24\columnwidth,height=!]{figs/npo_sam_df.pdf}
% \vspace*{-1mm}
% \\
% % \hspace*{2mm} {(a) Forget quality} & {(b) Model utility}
% \end{tabular}
% }
% \hspace*{21mm} \small{(a)} \hspace{31mm} \small{(b)} \\
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{cc}
% \hspace*{-3mm}
% \includegraphics[width=0.24\columnwidth,height=!]{figs/npo_gnr_df.pdf} 
% &
% \hspace*{-6mm}
% \includegraphics[width=0.24\columnwidth,height=!]{figs/npo_rs_df.pdf}
% \vspace*{-1mm}
% \\
% % \hspace*{2mm} {(a) Forget quality} & {(b) Model utility}
% \end{tabular}
% }
% \hspace*{21mm} \small{(c)} \hspace{31mm} \small{(d)}
% \vspace{-2mm}
% \caption{\small{Prediction loss landscape of the unlearned model obtained by NPO w/ or w/o smoothing over the WMDP Bio forget data. Z axis denotes the loss value.
% }}
% \label{fig: loss_landscape_df_diff_smooth}
% \vspace*{-5mm}
% \end{figure}


% % \begin{figure}[htb]
% % % \vspace*{-5mm}
% % \resizebox{\columnwidth}{!}{
% %     \includegraphics[width=0.28\columnwidth]{figs/method_step_wmdp_var.pdf}
% %     \includegraphics[width=0.28\columnwidth]{figs/method_epoch_wmdp_var.pdf}

% % }
% % % \vspace*{-6.5mm}
% % \caption{Performance of Relearning Attacks on NPO, GradDiff, and RMU w/o or w/ SAM. The figure format follows Fig.\,\ref{fig: relearn_wmdp_npo}.
% % }
% % \vspace*{-5mm}
% % \label{fig: relearn_wmdp_method}
% % \end{figure}

==> sections/methodology.tex <==
\section{Smoothness is the best companion of robustness}
\label{sec: method}
\begin{itemize}
    \item Utilize the loss landscape to demonstrate SAM can enhance the model's smoothness.
    \item SAM implicitly implements gradient norm regularization (Eq. 9 in \citep{dauphin2024neglected}).
    \item Sharpness is described as the trace of the Gauss-Newton matrix (Eq. 2 in \citep{dauphin2024neglected}). The Gauss-Newton matrix is a component of the Hessian matrix (Eq. 4 in \citep{dauphin2024neglected}).
    \item Further integration of other smoothing methods into the unlearning formulation, such as:
\end{itemize}

\noindent\textbf{Randomized Smoothing}
\begin{align}
    \minimize_{\boldsymbol{\theta}} \quad 
    \mathbb{E}_{(x, y) \in \Df, \boldsymbol{\epsilon} \sim \mathcal{N}(\mathbf{0},\sigma^{2}\mathbf{I})} \bigl[ \ellf(y | x; \boldsymbol{\theta} + \boldsymbol{\epsilon}) \bigr] \nonumber \\ 
    + \lambda \mathbb E_{(x, y) \in \Dr, \boldsymbol{\epsilon} \sim \mathcal{N}(\mathbf{0},\sigma^{2}\mathbf{I})} [ \ellr( y | x; \boldsymbol{\theta}) ]. \nonumber
\end{align}

\noindent\textbf{Gradient Norm Regularization}
\begin{align}
    \nonumber \displaystyle \minimize_{\boldsymbol{\theta}} \,\, \mathbb E_{(x, y) \in \Df} [ \ellf(y | x; \boldsymbol{\theta}) ] + \lambda \mathbb E_{(x, y) \in \Dr} [ \ellr( y | x; \boldsymbol{\theta}) ] \nonumber \\ 
    + \eta \|\nabla_{\boldsymbol{\theta}} \mathbb{E}_{(x, y) \in \mathcal{D}_f} [\ell_f(y | x; \boldsymbol{\theta})]\|_2 .
    \nonumber
\end{align}

\noindent\textbf{Weight Averaging}
\begin{align}
\boldsymbol{\theta}_{\text{SWA}}^{t} = \frac{\boldsymbol{\theta}_{\text{SWA}}^{t-1} \cdot n + \boldsymbol{\theta}^{t}}{n + 1}, \quad 
    \boldsymbol{\theta}^{t} = \boldsymbol{\theta}^{t-1} + \Delta \boldsymbol{\theta}^{t} . \nonumber
\end{align}


==> sections/outline.tex <==
\section{Outline}
\section{Introduction}
\section{Related work}
\begin{itemize}
    \item Overview of related work on LLM unlearning.
    \item Discussion of attacks and robustness in LLM unlearning, including relearning attacks, adversarial prompts, etc.
    \item Introduction to Sharpness-Aware Minimization (SAM) and other smoothing methods.
\end{itemize}

\section{Preliminary, motivation and problem statement}
\begin{itemize}
    \item Overview of LLM unlearning formulation.
    \item Relearning attacks can exploit a small number of samples for fine-tuning, enabling forgotten knowledge to reappear in the unlearned model. (Line Figure: Relearning Samples vs. WMDP Accuracy)
    \item The motivation is to ensure that the unlearned model is robust against relearning attacks and other attack methods.
\end{itemize}

\section{A robust optimization view on LLM unlearning and relearning}
\begin{itemize}
    \item Adversarial training can be introduced into LLM unlearning. Interestingly, the SAM formulation aligns with the min-max formulation of adversarial training.
    \begin{itemize}
        \item In the outer loop, we minimize the forget loss and retain loss to achieve unlearning.
        \item In the inner loop, we maximize the forget loss, simulating relearning attacks to encourage the model to relearn forgotten knowledge.
    \end{itemize}
    \noindent\textbf{Sharpness-Aware Minimization:}
    \begin{align}
        \begin{array}{l}
         \displaystyle \minimize_{\boldsymbol{\theta}} \,\, \mathbb E_{(x, y) \in \Df} [ \ellf(y | x; \boldsymbol{\theta} + \boldsymbol{\epsilon}^*)] + \lambda \mathbb E_{(x, y) \in \Dr} [ \ellr( y | x; \boldsymbol{\theta}) ], \nonumber \\
        \text{where} \quad \boldsymbol{\epsilon}^* = \arg\max_{\|\boldsymbol{\epsilon}\|_2 \leq \rho} \mathbb E_{(x, y) \in \Df} \ellf(y | x; \boldsymbol{\theta} + \boldsymbol{\epsilon}).
        \end{array}
    \end{align}
\end{itemize}


\section{Smoothness is the best companion of robustness}
\begin{itemize}
    \item Utilize the loss landscape to demonstrate SAM can enhance the model's smoothness.
    \item SAM implicitly implements gradient norm regularization (Eq. 9 in \citep{dauphin2024neglected}).
    \item Sharpness is described as the trace of the Gauss-Newton matrix (Eq. 2 in \citep{dauphin2024neglected}). The Gauss-Newton matrix is a component of the Hessian matrix (Eq. 4 in \citep{dauphin2024neglected}).
    \item Further integration of other smoothing methods into the unlearning formulation, such as:
    \begin{itemize}
        \item \textbf{Randomized Smoothing}
        \begin{align}
            \minimize_{\boldsymbol{\theta}} \quad 
            \mathbb{E}_{(x, y) \in \Df, \boldsymbol{\epsilon} \sim \mathcal{N}(\mathbf{0},\sigma^{2}\mathbf{I})} \bigl[ \ellf(y | x; \boldsymbol{\theta} + \boldsymbol{\epsilon}) \bigr] \nonumber \\ 
            + \lambda \mathbb E_{(x, y) \in \Dr, \boldsymbol{\epsilon} \sim \mathcal{N}(\mathbf{0},\sigma^{2}\mathbf{I})} [ \ellr( y | x; \boldsymbol{\theta}) ] \nonumber
        \end{align}
        \item \textbf{Gradient Norm Regularization}
        \begin{align}
            \nonumber \displaystyle \minimize_{\boldsymbol{\theta}} \,\, \mathbb E_{(x, y) \in \Df} [ \ellf(y | x; \boldsymbol{\theta}) ] + \lambda \mathbb E_{(x, y) \in \Dr} [ \ellr( y | x; \boldsymbol{\theta}) ] \nonumber \\ 
            + \eta \|\nabla_{\boldsymbol{\theta}} \mathbb{E}_{(x, y) \in \mathcal{D}_f} [\ell_f(y | x; \boldsymbol{\theta})]\|_2
            \nonumber
        \end{align}
        \item \textbf{Weight Averaging}
        \begin{align}
        \boldsymbol{\theta}_{\text{SWA}}^{t} = \frac{\boldsymbol{\theta}_{\text{SWA}}^{t-1} \cdot n + \boldsymbol{\theta}^{t}}{n + 1}, \quad 
            \boldsymbol{\theta}^{t} = \boldsymbol{\theta}^{t-1} + \Delta \boldsymbol{\theta}^{t} \nonumber
        \end{align}
    \end{itemize}
\end{itemize}

\section{Experiments}
\subsection{Performance on the WMDP Benchmark}
\begin{itemize}
    \item Evaluate robustness under two different relearning settings (\textbf{Table\,\ref{tab: relearn_wmdp}} + \textbf{Fig.\,\ref{fig: relearn_wmdp_npo}} + \textbf{Fig.\,\ref{fig: relearn_wmdp_method}} + loss landscape)
        \begin{itemize}
            \item Same number of relearning samples but with different relearning epochs.
            \item Different numbers of relearning samples with the same relearning epoch.
        \end{itemize} 
    \item Combining different smoothing methods with unlearning methods improves model robustness.
    \item Robustness of unlearning method NPO $>$ GradDiff $>$ RMU
\end{itemize}

\subsection{Performance on the MUSE Benchmark}
\subsection{Robustness to adversarial prompt}
\begin{itemize}
    \item Use shallow safety issues in unlearning to elaborate.
    \item Demonstrate that smoothness can also enhance robustness against input-space attacks, such as jailbreak prompts.
\end{itemize}
\subsection{Investigating the mismatch between unlearning, relearning, and smoothing on the dataset.} 

\begin{table*}[t]
\caption{Unlearning and Relearning Performance on WMDP Bio. Relearning attacks are conducted using WMDP Bio, AGNews, GSM8K, and SST2. $\blacktriangle$ indicates that the higher the metric, the better. The performance gap in WMDP Bio Acc before and after the relearning attack is indicated by (\textcolor{blue}{$\bullet$}). Note that a smaller performance gap compared to the \textit{"Before Attack"} accuracy reflects better robustness of the MU method. The metric \textit{Avg.} is calculated as the average 1 - WMDP Bio Acc, including WMDP Bio, AGNews, GSM8K, and SST2.}

\label{tab: relearn_wmdp}
\begin{center}
\begin{tabular}{c|c|c|cccc|c}
\toprule[1pt]
\midrule
\multirow{3}{*}{Method} & \multirow{3}{*}{MMLU ($\blacktriangle$)} & \multicolumn{6}{c}{1 - WMDP Bio Acc ($\blacktriangle$)} \\                             & & Before Attack & WMDP Bio & AGNews & GSM8K & SST2 & Avg. \\
\midrule
\rowcolor{Gray}
\multicolumn{8}{c}{\textbf{20 samples for 3 epochs}} \\
\midrule
NPO       & 0.44 & 0.74 & 0.37 (\textcolor{blue}{0.36}) & 0.39 (\textcolor{blue}{0.35}) & 0.38 (\textcolor{blue}{0.36}) & 0.38 (\textcolor{blue}{0.36}) & 0.38 (\textcolor{blue}{0.36}) \\
\midrule
NPO + SAM & 0.42 & 0.74 & 0.59 (\textcolor{blue}{0.15}) & 0.41 (\textcolor{blue}{0.33}) & 0.42 (\textcolor{blue}{0.32}) & 0.41 (\textcolor{blue}{0.32}) & 0.46 (\textcolor{blue}{0.28}) \\
NPO + RS  & 0.41 & 0.74 & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.33}) & 0.42 (\textcolor{blue}{0.32}) \\
NPO + GNR & 0.45 & 0.73 & 0.43 (\textcolor{blue}{0.30}) & 0.40 (\textcolor{blue}{0.33}) & 0.45 (\textcolor{blue}{0.28}) & 0.49 (\textcolor{blue}{0.24}) & 0.44 (\textcolor{blue}{0.29}) \\
NPO + SWA & 0.46 & 0.74 & 0.43 (\textcolor{blue}{0.30}) & 0.39 (\textcolor{blue}{0.34}) & 0.39 (\textcolor{blue}{0.35}) & 0.39 (\textcolor{blue}{0.34}) & 0.40 (\textcolor{blue}{0.33}) \\
\midrule
\rowcolor{Gray}
\multicolumn{8}{c}{\textbf{60 samples for 1 epoch}} \\
\midrule
NPO       & 0.44 & 0.74 & 0.37 (\textcolor{blue}{0.37}) & 0.39 (\textcolor{blue}{0.35}) & 0.37 (\textcolor{blue}{0.37}) & 0.38 (\textcolor{blue}{0.36}) & 0.38 (\textcolor{blue}{0.36}) \\
\midrule
NPO + SAM & 0.42 & 0.74 & 0.45 (\textcolor{blue}{0.29}) & 0.42 (\textcolor{blue}{0.32}) & 0.42 (\textcolor{blue}{0.32}) & 0.43 (\textcolor{blue}{0.31}) & 0.43 (\textcolor{blue}{0.31}) \\
NPO + RS  & 0.41 & 0.74 & 0.41 (\textcolor{blue}{0.33}) & 0.41 (\textcolor{blue}{0.33}) & 0.41 (\textcolor{blue}{0.33}) & 0.40 (\textcolor{blue}{0.34}) & 0.41 (\textcolor{blue}{0.33}) \\
NPO + GNR & 0.45 & 0.73 & 0.43 (\textcolor{blue}{0.30}) & 0.48 (\textcolor{blue}{0.25}) & 0.50 (\textcolor{blue}{0.23}) & 0.49 (\textcolor{blue}{0.24}) & 0.47 (\textcolor{blue}{0.25}) \\
NPO + SWA & 0.46 & 0.74 & 0.40 (\textcolor{blue}{0.34}) & 0.42 (\textcolor{blue}{0.32}) & 0.39 (\textcolor{blue}{0.34}) & 0.40 (\textcolor{blue}{0.34}) & 0.40 (\textcolor{blue}{0.34}) \\
\midrule
\bottomrule[1pt]
\end{tabular}
\end{center}
\end{table*}

\begin{figure}[htb]
% \vspace*{-5mm}
\resizebox{\columnwidth}{!}{
    \includegraphics[width=0.28\columnwidth]{figs/npo_step_wmdp_var.pdf}
    \includegraphics[width=0.28\columnwidth]{figs/npo_epoch_wmdp_var.pdf}

}
\vspace*{-6.5mm}
\caption{Performance of Relearning Attacks on NPO w/o or w/ Smoothing. The evaluation is conducted under two relearning settings: (a) varying the number of relearning samples (20, 40, 60) with the same number of relearning epochs (1), and (b) fixing the number of relearning samples (20) while varying the number of relearning epochs (1, 2, 3). The results are averaged over five independent random trials.
}
% \vspace*{-5mm}
\label{fig: relearn_wmdp_npo}
\end{figure}

\begin{figure}[htb]
% \vspace*{-5mm}
\resizebox{\columnwidth}{!}{
    \includegraphics[width=0.28\columnwidth]{figs/method_step_wmdp_var.pdf}
    \includegraphics[width=0.28\columnwidth]{figs/method_epoch_wmdp_var.pdf}

}
% \vspace*{-6.5mm}
\caption{Performance of Relearning Attacks on NPO, GradDiff, and RMU w/o or w/ SAM. The figure format follows Fig.\,\ref{fig: relearn_wmdp_npo}.
}
\vspace*{-5mm}
\label{fig: relearn_wmdp_method}
\end{figure}


==> sections/preliminary.tex <==
\section{Preliminary, motivation and problem statement}
\label{sec: preliminary}
\begin{itemize}
    \item Overview of LLM unlearning formulation.
    \item Relearning attacks can exploit a small number of samples for fine-tuning, enabling forgotten knowledge to reappear in the unlearned model. (Line Figure: Relearning Samples vs. WMDP Accuracy)
    \item The motivation is to ensure that the unlearned model is robust against relearning attacks and other attack methods.
\end{itemize}

\section{A robust optimization view on LLM unlearning and relearning}
\begin{itemize}
    \item Adversarial training can be introduced into LLM unlearning. Interestingly, the SAM formulation aligns with the min-max formulation of adversarial training.
    \begin{itemize}
        \item In the outer loop, we minimize the forget loss and retain loss to achieve unlearning.
        \item In the inner loop, we maximize the forget loss, simulating relearning attacks to encourage the model to relearn forgotten knowledge.
    \end{itemize}
\end{itemize}

\noindent\textbf{Sharpness-Aware Minimization:}
\begin{align}
     \min_{\boldsymbol{\theta}} \left\{\ \max_{\|\boldsymbol{\epsilon}\|_2 \leq \rho} \mathbb{E}_{(x,y)\in \Df}\left[\ellf(y| x; \boldsymbol{\theta} + \boldsymbol{\epsilon})\right] + \lambda \mathbb{E}_{(x,y)\in \mathcal{D}_r}\left[\ellr(y| x; \boldsymbol{\theta})\right] \right\}. \nonumber
\end{align}
